GPU Accelerated Sub-Sampled Newton's Method

First order methods, which solely rely on gradient information, are commonly used in diverse machine learning (ML) and data analysis (DA) applications. This is attributed to the simplicity of their implementations, as well as low per-iteration computational/storage costs. However, they suffer from significant disadvantages; most notably, their performance degrades with increasing problem ill-conditioning. Furthermore, they often involve a large number of hyper-parameters, and are notoriously sensitive to parameters such as the step-size. By incorporating additional information from the Hessian, second-order methods, have been shown to be resilient to many such adversarial effects. However, these advantages of using curvature information come at the cost of higher per-iteration costs, which in \enquote{big data} regimes, can be computationally prohibitive. In this paper, we show that, contrary to conventional belief, second-order methods, when implemented appropriately, can be more efficient than first-order alternatives in many large-scale ML/ DA applications. In particular, in convex settings, we consider variants of classical Newton\textsf{'}s method in which the Hessian and/or the gradient are randomly sub-sampled. We show that by effectively leveraging the power of GPUs, such randomized Newton-type algorithms can be significantly accelerated, and can easily outperform state of the art implementations of existing techniques in popular ML/ DA software packages such as TensorFlow. Additionally these randomized methods incur a small memory overhead compared to first-order methods. In particular, we show that for million-dimensional problems, our GPU accelerated sub-sampled Newton\textsf{'}s method achieves a higher test accuracy in milliseconds as compared with tens of seconds for first order alternatives.

==> tex/softmax.tex <==
For completeness, we now briefly review multi-class classification using soft-max and cross-entropy loss function, as an important instance of the problems of the form~\eqref{eq:obj}. Consider $ p $ dimensional feature vector $ \aa $, and the corresponding label $ b $ which can belong to one of $C$ classes. In such a classifier, the probability that $\aa$ belongs to a class $c \in \{1,2,\ldots,C\}$ is given as
\begin{align*}
\Pr\left(b = c \mid \aa,\xx_{1},\ldots, \xx_{C}\right) = \frac{e^{\lin{\aa,\xx_{c}}}}{\sum_{c' = 1}^{C} e^{\lin{\aa, \xx_{c'}}}},
\end{align*}
where $ \xx_{c} \in \mathbb{R}^{p}$ is the weight vector corresponding to class $ c $. Recall that here there are only $ C-1 $ degrees of freedom, i.e., probabilities all must sum to one. Consequently, for a training data $\{\aa_{i},b_{i}\}_{i=1}^{n} \subset \mathbb{R}^{p} \times \{1,2,\ldots,C\}$, the cross-entropy loss function for $ \xx = [\xx_{1}; \xx_{2}; \ldots; \xx_{C-1}] \in \mathbb{R}^{(C-1)p} $ can be written as
\begin{align}
\label{eq:softmax_log_likelihood}
&F(\xx) \triangleq F(\xx_{1},\xx_{2},\ldots,\xx_{C-1}) \nonumber \\
= &\sum_{i=1}^{n} \left(\log \left(1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}\right)  - \sum_{c = 1}^{C-1}\mathbf{1}(b_{i} = c) \lin{\aa_{i},\xx_{c}}\right).
\end{align} 
Note that here $ d = (C-1) p $. It then follows that the gradient of $f$ with respect to $\xx_c$ is
\begin{align}
\label{eq:softmax_gradient}
\nabla_{\xx_{c}} F(\xx) = \sum_{i=1}^{n} \left(\frac{e^{\lin{\aa_{i}, \xx_{c}}}}{1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}}  - \mathbf{1}(b_{i} = c) \right) \aa_{i}.
\end{align}
Similarly  for the Hessian, we have
\begin{subequations}
	\label{eq:softmax_hessian}
	\begin{flalign}
	& \nabla^{2}_{\xx_{c},\xx_{c}} F = \nonumber \\ 
	& \sum_{i=1}^{n} \left(\frac{e^{\lin{\aa_{i}, \xx_{c}}}}{1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}} - \frac{e^{2\lin{\aa_{i}, \xx_{c}}}}{\left(1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}\right)^{2}} \right) \aa_{i} \aa_{i}^{T},  \label{eq:softmax_hessian_wc_wc}
	\end{flalign}
	and for $ \hat{c} \in \{1,2,\ldots,C-1\} \setminus \{c\} $, we get
	\begin{flalign}
	& \nabla^{2}_{\xx_{c},\xx_{\hat{c}}} F = \sum_{i=1}^{n} \left(- \frac{e^{\lin{\aa_{i}, \xx_{\hat{c}} + \xx_{c}}}}{\left(1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}\right)^{2}} \right) \aa_{i} \xx_{i}^{T} 	\label{eq:softmax_hessian_wc_wb}. 
	\end{flalign}
\end{subequations}

\subsubsection{Numerical Stability}
\label{sec:numerical_stability}
To avoid over-flow in the evaluation of exponential functions, we use the ``Log-Sum-Exp'' trick~\cite{murphy2012machine}. Specifically, for each data point $\aa_{i}$, we first find the maximum value among $\lin{\aa_{i},\xx_{c}}, \; c=1,\ldots, C-1$. Define
\begin{align}
\label{eq:max_x}
M(\aa) = \max \Big\{ 0, \lin{\aa,\xx_{1}}, \lin{\aa,\xx_{2}}, \ldots, \lin{\aa,\xx_{C-1}} \Big\}, 
\end{align}
and 
\begin{align}
\label{eq:log_sum_trick}
\alpha(\aa) \defeq e^{-M(\aa)}+\sum_{c' = 1}^{C-1} e^{\lin{\aa, \xx_{c'}} - M(\aa)}.
\end{align}
Note that $M(\aa) \geq0, \alpha(\aa) \geq 1$. Now, we have

\begin{align*}
1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}} 
%& = e^{M(\aa_{i})} \left(e^{-M(\aa_{i})}+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}} - M(\aa_{i})}\right) \\
& = e^{M(\aa_{i})} \alpha(\aa_{i}).
\end{align*}
So for computing~\eqref{eq:softmax_log_likelihood}, we do
\begin{align*}
& \log \left(1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}\right) \\
&= M(\aa_{i}) + \log \left(e^{-M(\aa_{i})}+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}} - M(\aa_{i})}\right) \\
&= M(\aa_{i}) + \log \big( \alpha(\aa_{i}) \big).
\end{align*}
Similarly, for~\eqref{eq:softmax_gradient} and~\eqref{eq:softmax_hessian}, we can use
\begin{align*}
\frac{e^{\lin{\aa_{i}, \xx_{c}}}}{1+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}}}} &= \frac{e^{\lin{\aa_{i}, \xx_{c}}-M(\aa_{i})}}{e^{-M(\aa_{i})}+\sum_{c' = 1}^{C-1} e^{\lin{\aa_{i}, \xx_{c'}} - M(\aa_{i})}} \\
&= \frac{e^{\lin{\aa_{i}, \xx_{c}}-M(\aa_{i})}}{\alpha(\aa_{i})}.
\end{align*}

Note that is all these computations, we are always guaranteed to have all the exponents appearing in all the exponential functions to be negative, hence avoiding numerical over-flow.
%Another less reliable but simpler approach is to note that since all~\eqref{eq:softmax_log_likelihood},~\eqref{eq:softmax_gradient}, and~\eqref{eq:softmax_hessian} are shift invariant, we can pre-process the original data set to $X_{i,j} \leftarrow \left(X_{i,j} - M\right), \; \forall i,j$ and work with this new data set. The value of the shift can be $M = \|X\|_{\infty}$ or $M = \max_{i}\{ \|\aa_{i}\|_{2} \}$, among others.

\subsubsection{Hessian Vector Product}
\label{sec:MVP}
For a vector $\vv^{T} = [\vv_{1}^{T},\vv_{2}^{T},\ldots,\vv_{C-1}^{T}]^{T}$, we can compute the Hessian-vector product without explicitly forming the Hessian. Let us for notational simplicity define
\begin{align*}
\stepcounter{equation}\tag{\theequation}\label{eq:hxw}
h(\aa,\xx) \defeq \frac{e^{\lin{\aa, \xx}-M(\xx)}}{\alpha(\aa)}, 
\end{align*}
where $M(\xx)$ and $ \alpha(\xx) $ were defined in~\eqref{eq:max_x} and~\eqref{eq:log_sum_trick}, respectively.
Now using matrices 
\begin{align*}
\stepcounter{equation}\tag{\theequation}\label{eq:matrix-a}
\V = \begin{bmatrix}
\lin{\aa_{1},\vv_{1}} & \lin{\aa_{1},\vv_{2}} & \dots  & \lin{\aa_{1},\vv_{C-1}} \\
\lin{\aa_{2},\vv_{1}} & \lin{\aa_{2},\vv_{2}} & \dots  & \lin{\aa_{2},\vv_{C-1}} \\
\vdots & \vdots & \ddots & \vdots \\
\lin{\aa_{n},\vv_{1}} & \lin{\aa_{n},\vv_{2}} & \dots  & \lin{\aa_{n},\vv_{(C-1)}}
\end{bmatrix}_{n \times (C-1)}, %\label{eq:matrix-a}
\end{align*}
and
\begin{align*}
\stepcounter{equation}\tag{\theequation}\label{eq:matrix-b}
\W = \begin{bmatrix}
h(\aa_{1},\xx_{1}) & h(\aa_{1},\xx_{2}) & \dots  & h(\aa_{1},\xx_{C-1}) \\
h(\aa_{2},\xx_{1}) & h(\aa_{2},\xx_{2}) & \dots  & h(\aa_{2},\xx_{C-1}) \\
\vdots & \vdots & \ddots & \vdots \\
h(\aa_{n},\xx_{1}) & h(\aa_{n},\xx_{2}) & \dots  & h(\aa_{n},\xx_{C-1}) \\
\end{bmatrix}_{n \times (C-1)},
\end{align*}
we compute
\begin{align*}
\stepcounter{equation}\tag{\theequation}\label{eq:matrix-c}
\U = \V \odot \W - \W \odot \Big( \big(\left(\V \odot \W\right) \ee \big) \ee^{T} \Big), 
\end{align*}
to get
\begin{align*}
\stepcounter{equation}\tag{\theequation}\label{eq:hessianvec}
\H\vv = \text{vec} \left( \A^{T} \U \right), 
\end{align*}
where $\ee \in \mathbb{R}^{C-1}$ is a vector of all $1$'s, and each row of the matrix $ \A \in \mathbb{R}^{n \times p}$ is a row vector corresponding to the $i^{th}$ data point, i.e, $\A^{T} = \begin{bmatrix} \aa_{1}, \aa_{2}, \ldots, \aa_{n} \end{bmatrix}$.




